Multi-line observations of CH$_{3}$OH, c-C$_{3}$H$_{2}$ and HNCO towards L1544: Dissecting the core structure with chemical differentiation

Pre-stellar cores are the basic unit for the formation of stars and stellar systems. The anatomy of the physical and chemical structures of pre-stellar cores is critical for understanding the star formation process. L1544 is a prototypical pre-stellar core, which shows significant chemical differentiation surrounding the dust peak. We aim to constrain the physical conditions at the different molecular emission peaks. This study allows us to compare the abundance profiles predicted from chemical models together with the classical density structure of Bonnor-Ebert (BE) sphere. We conducted multi-transition pointed observations of CH$_{3}$OH, c-C$_{3}$H$_{2}$ and HNCO with the IRAM 30m telescope, towards the dust peak and the respective molecular peaks of L1544. With non-LTE radiative transfer calculations and a 1-dimensional model, we revisit the physical structure of L1544, and benchmark with the abundance profiles from current chemical models. We find that the HNCO, c-C$_{3}$H$_{2}$ and CH$_{3}$OH lines in L1544 are tracing progressively higher density gas, from $\sim$10$^{4}$ to several times 10$^{5}$ cm$^{-3}$. Particularly, we find that to produce the observed intensities and ratios of the CH$_{3}$OH lines, a local gas density enhancement upon the BE sphere is required. This suggests that the physical structure of an early-stage core may not necessarily follow a smooth decrease of gas density profile locally, but can be intercepted by clumpy substructures surrounding the gravitational center. Multiple transitions of molecular lines from different molecular species can provide a tomographic view of the density structure of pre-stellar cores. The local gas density enhancement deviating from the BE sphere may reflect the impact of accretion flows that appear asymmetric and are enhanced at the meeting point of large-scale cloud structures.

==> tab1_addbeam.tex <==
\begin{tabular}{lrrrl}
\toprule
                     0 &        1 &    2 &     3 &     4 \\
\midrule
 2$_{-1,2}$-1$_{-1,1}$ &  96.7394 & 12.5 &  1.30 &  26.0 \\
   2$_{0,2}$-1$_{0,1}$ &  96.7445 & 20.1 & 15.40 &  26.0 \\
   2$_{1,2}$-1$_{1,1}$ &  96.7555 & 28.0 & 31.50 &  26.0 \\
   3$_{0,3}$-2$_{0,2}$ & 145.0938 & 27.1 & 26.20 &  17.3 \\
 3$_{-1,3}$-2$_{-1,2}$ & 145.0974 & 19.5 &  4.40 &  17.3 \\
   3$_{1,3}$-2$_{1,2}$ & 145.1319 & 35.0 & 46.10 &  17.3 \\
  4$_{0,4}$-4$_{-1,4}$ & 157.2461 & 36.3 & 44.20 &  16.0 \\
  1$_{0,1}$-1$_{-1,1}$ & 157.2708 & 15.4 &  9.30 &  16.0 \\
  3$_{0,3}$-3$_{-1,3}$ & 157.2723 & 27.1 & 26.20 &  16.0 \\
  2$_{0,2}$-2$_{-1,2}$ & 157.2760 & 20.1 & 15.30 &  16.0 \\
   3$_{0,3}$-2$_{0,2}$ & 145.1032 & 13.9 &  3.95 &  17.3 \\
   3$_{1,2}$-2$_{2,1}$ & 145.0896 & 16.1 & 10.40 &  17.3 \\
   3$_{3,0}$-2$_{2,1}$ & 216.2788 & 19.5 & 33.70 &  11.6 \\
   6$_{1,6}$-5$_{0,5}$ & 217.8221 & 38.6 & 70.80 &  11.5 \\
   4$_{3,2}$-3$_{2,1}$ & 227.1691 & 29.1 & 52.00 &  11.1 \\
   5$_{0,5}$-4$_{0,4}$ & 109.9058 & 15.8 &  5.10 &  22.9 \\
   6$_{0,6}$-5$_{0,5}$ & 131.8857 & 22.1 &  8.80 &  19.1 \\
   7$_{0,7}$-6$_{0,6}$ & 153.8651 & 29.5 & 13.90 &  16.3 \\
   8$_{0,8}$-7$_{0,7}$ & 175.8437 & 38.0 & 21.50 &  14.3 \\
\bottomrule
\end{tabular}

